Impact of 3D macro physics and nuclear physics on the p nuclei in O-C shell mergers

O-C shell mergers in massive stars are a site for producing the p nuclei by the $\gamma$ process, but 1D stellar models rely on mixing length theory, which does not match the radial velocity profiles of 3D hydrodynamic simulations. We investigate how 3D macro physics informed mixing impacts the nucleosynthesis of p nuclei. We post-process the O-shell of the $M_\mathrm{ZAMS} = 15~\mathrm{M}_\odot$, $Z = 0.02$ model from the NuGrid stellar data set. Applying a downturn to velocities at the boundary and increasing velocities across the shell as obtained in previous results, we find non-linear, non-monotonic increase in p-nuclei production with a spread of 0.96 dex, and find that isotopic ratios can change. Reducing C-shell ingestion rates as found in 3D simulations suppresses production, with spreads of 1.22-1.84 dex across MLT and downturn scenarios. Applying dips to the diffusion profile to mimic quenching events also suppresses production, with a 0.51 dex spread. We analyze the impact of varying all photo-disintegration rates of unstable n-deficient isotopes from Se-Po by a factor of 10 up and down. The nuclear physics variations for the MLT and downturn cases have a spread of 0.56-0.78 dex. We also provide which reaction rates are correlated with the p nuclei, and find few correlations shared between mixing scenarios. Our results demonstrate that uncertainties in mixing arising from uncertain 3D macro physics are as significant as nuclear physics and are crucial for understanding p-nuclei production during O-C shell mergers quantitatively.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
\newcommand{\vort}{\ensuremath{|\curl u|}}
\newcommand{\vortsq}{\ensuremath{\vort^2}}
% end vectors.tex

